Toward Mining Visual Log of Software

In this paper, we define visual log of a software system as data capturing the interactions between its users and its graphic user interface (GUI), such as screen-shots and screen recordings. We vision that mining such visual log could be useful for bug reproducing and debugging, automated GUI testing, user interface designing, question answering of common usages in software support, etc. Toward that vision, we propose a core framework for mining visual log of software. This framework focuses on detecting GUI elements and changes in visual log, removing users' private data, recognizing user interactions with GUI elements, and learning GUI usage patterns. We also performed a small study on the characteristics of GUI elements in mobile apps. The findings from this study suggested several heuristics to design techniques for recognizing GUI elements and interactions.

==> proposal.tex <==
\section{Future directions}

Once we collects multiple user interaction sequences we could then start the learning phrase. We could use a generative model to capture the interaction sequences such as a Hidden Markov Model or a Recurrent Neural Network. Such models (once learned) will enable us to generate new interaction sequences that have similar characteristic of the originals. One of the application of such model is test case generation. For example, visual logs were collected during human testing of an application, these test were conduct by tester interact with the application base on several scenarios. The visual logs collected will then be used to generate extra test case that have the same characteristic as original scenarios. These test cases (new generated user interactions) and origin test sequences (extracted by our system) will be used for automatic testing in a continuous integration system.



==> researchQ.tex <==
\begin{table}[t!]
	\centering
	\tt\scriptsize
	\caption{Empirical study data}
	\begin{tabular}{lrrrrrr}
		\toprule
		\textbf{Device}   & Experiments & Sampled Frames & Labeled Objects\\
		\midrule
		iPhone 5s & 10         & 70          & 957 \\
		iPhone 6  & 10         & 63          & 904 \\
        iPhone 6p & 10         & 67          & 943 \\
		\bottomrule
	\end{tabular}
	\label{tab:datastat}
\end{table}

\begin{table}[t!]
	\centering
	\tt\scriptsize
	\caption{Shapes of Icon and Combine elements}
	\begin{tabular}{@{}p{20pt}R{38pt}R{26pt}R{22pt}R{17pt}R{21pt}R{38pt}@{}}
		\toprule
		\textbf{Type}& Rectangle & Circle & Arrow  & Tick  & Cross & Irregular \\
		\midrule
		Icon 		 & 21.7\%    & 9.6\%  & 10.6\% & 8.0\% & 8.3\% & 41.8\%\\
		Combine	 	 & 41.3\%    & 46.7\% &        &       &       & 12.1\%\\
		\bottomrule
	\end{tabular}
	\label{tab:typeShape}
\end{table}

\section{Empirical study}
To help in design those algorithms, we perform an empirical study to understand the characteristics of GUI elements. We limit the scope of our studies to photo apps for mobile phones. The study was carried on data collected from two major photo editing applications: Camera 360 and Photo Wonder. Table~\ref{tab:datastat} shows the details of the data used. A set of videos were recorded while the user interact with the two applications on three different phone size (iPhone 6 Plus, 6, and 5s). A Major Event detector was used to detect if a page change has happen (a large spike in the square mean error between to consecutive frames). When such major event occurs, a sample frame will be taken after some delay, the purpose of this technique is to sample most of the distinct UI screens while trying to prevent sampling the same UI screen multiple time. Table~\ref{tab:datastat} shows that we sampled on average 6 to 7 frames per experiments while each of those frame contains on average 14 labeled visual objects.

Each of the above sampled frames were inspected manually by three PhD students. These students labeled object that are considered user interface element and decide which type it is: Text (Textual content), Icon (An image or drawing that indicate an intractable functionality), or Combine (An user interface element that might contain Text, Icon, or other Combine). The students also determine the shape (Rectangle, Circle, Triangle, Arrow, Tick, Cross, or Irregular) and orientation (Horizontal, Vertical, or Irregular) of each user interface element . They also indicate the relation between close by elements (e.g. An explanatory text below an icon, these two are considered related).

For example, on the top left corner of Figure~\ref{fig:detectFlow} is the home screen of Camera 360 on an iPhone 6 Plus, we can see the three types of element in one single button. The button Camera is a Combine element which contain an Icon element (camera drawing) and an Text element (the word Camera). The camera Icon and Text are related to the Combine button and their relative position is inside.

\todo{Explain what we study}

From our data analysis, most of the elements are Text at 48.3~\% and Icon at 39.4~\%. This might suggest that for mobile application (in such a small display area) elements can just be word(s) or a simple small image or drawing and it is not efficient to create bounding and combine them into Combine elements. Most of the 12.3\% Combine elements are big buttons on the home screen or some slides created to enable user to adjust certain image properties.

\todo{Rewrite in term of heuristic}
\begin{enumerate}  
\item Filter too small contours ( UI elements need to be a certain size for user to see and interact) \todo{get limit in element size}
\item Combine outer and inner contours of the same object (after dilation an object will have two contours of the same thick border, these needed to be combined to prevent duplication in object detection) \todo{technique artifact}
\item Filter contours with irregular shapes (not circle or rectangle) if above a certain bounding size (indicating it is not likely an Icon) \todo{shape, size}
\item Filter contours with irregular orientation (not horizontal or vertical) if above a certain bounding size (indicating it is not likely an Icon) \todo{orientation, size}
\item Relative position text and icon and combine \todo{text to the right and below icon, always aligned}
\end{enumerate}

Table~\ref{tab:typeShape} shows the different shapes Icon and Combine elements could have. Icon elements are variety in shape, most of them are Irregular (41.8\%) and Rectangle (21.7\%). The rest are divided equally among other shapes: Arrow at 10.6\%, Circle at 9.6\%, Tick at 8.0\%, and Cross at 8.3\%. This result show that the shapes of an Icon can be anything.

We also verified that all Text element are arranged horizontally, while 98.1\% of Icons are placed horizontally, 9\% of them are vertically placed, and 22\% are not either horizontal or vertical. This again confirms that Icon can be of any shape and they could be place in any angle. On the other hand, Combines are all either horizontal (87\%) or vertical(12.7\%). This mean that compounded UI element are place in alignment  with the screen and hence with others.

The experiment was done on three screen size iPhone 5s (small: 1136 x 640), iPhone 6 (medium: 1334 x 750), and iPhone 6 Plus (large: 1920 x 1080). Each element bounding box was calculated and the ratio of these bounding boxes area with respect to the actual screen area was calculated. Figure~\ref{fig:areaRatioExperiment} shows the ratios of different types of element (Text, Icon, and Combine) in respect to the screen sizes were used. We can see that for textual element the ratio are decreasing as the screen getting larger. This is because user feel comfortable with a certain size of font and increase the font size with the increase of screen size would make the text harder to read and the application would look proportionally incorrect. Between the two applications Camera 360 have a more consistence font size than Photo Wonder, this is the design choice that the developer make but they are not too far apart. 

On the other hand elements of type Icon have a more consistence ratio across screen size, this is because they are simply scaled up to the corresponding screen size to make the layout look consistent. There are minimum differences between the two applications. As for element of type Combine, we can see that they are scaled down similarly to textual element with similar scale rate as well (Camera 360 have more consistent absolute size than Photo Wonder), however between the two applications, the sizes of combination are vastly different. Photo Wonder has much bigger Combine elements (Buttons, slides) where as elements of the same type in Photo Wonder have significantly smaller sizes. We can see two different design style in these two applications.

\begin{figure}[t!]
	\centering
	%\tt\scriptsize
	\includegraphics[width=0.45\textwidth]{Data/T_Ratio_Combine.pdf}
	\includegraphics[width=0.45\textwidth]{Data/I_Ratio_Combine.pdf}
	\includegraphics[width=0.45\textwidth]{Data/C_Ratio_Combine.pdf}
	\caption{Ratios of element areas with respect to screen area and application.}
	
	\label{fig:areaRatioExperiment}
\end{figure}

\todo{We cannot get the stat about how many icon or combination have related Text. We can only have the stat on how many text are not related to anything, or how many icon are not related to anything. The stat for combine is not correct... since we do not count the inside relationship for this type... What should we get for this}

\todo{percentage of text label not related to anything}
\todo{percentage of icon not related to anything}
\todo{percentage of icon, label related to Combine that are inside...}

Of all textual label that explain an Icon, 79.2\% are below while (17.4\%) of them are on the right of such Icon. There are 3.4\% of the time the label is on the left of the Icon it is explaining, this is the case where the label explaining for an arrow that is pointing right (control functions such as forward, next...) This shows a common pattern that is in order to include textual label explaining meaning of Icon element that represent certain functionality, they are commonly put bellow or on the right in a natural flow of reading. While most of Combine elements have related Textual labels bellow (48\%) and inside (47\%). Only 4.5\% of the related Text elements are on the left of Combine elements, these are mostly labels for the slices to adjust some image properties. In all of the cases, the related text are close to the Icons or Combines they are explaining and in vertical or horizontal alignment with such Icons or Combines.



--- store text

\begin{figure}[t!]
	\centering
	%\tt\scriptsize
	\includegraphics[width=0.4\textwidth]{Data/T_Ratio_Combine.pdf}
	\includegraphics[width=0.4\textwidth]{Data/I_Ratio_Combine.pdf}
	\includegraphics[width=0.4\textwidth]{Data/C_Ratio_Combine.pdf}
	\caption{Relative size of GUI elements (vs screen size)}
	
	\label{fig:areaRatioExperiment}
\end{figure}

\section{Empirical study}

To design the algorithms for detecting GUI elements and user interactions, we performed a preliminary empirical study on the characteristics of GUI elements. We limit the scope of this study to photo apps for mobile phones because i) they would have the most intuitive and easy-to-use GUI and ii) their user base would be very large and highly diverse. We selected two apps \code{Camera 360} and \code{Photo Wonder} for this study.

\subsection{Data collection}

We designed 10 photo editing tasks and performed them in those two apps on three different phone models (iPhone 6 Plus, 6, and 5s, each has a different screen size). While performing editing tasks, we recorded the screen of those apps. After that, we extracted screen shots (i.e. frames) from the recorded videos when major GUI events happened (e.g. clicking in a button or a list item) and selected a random sample of those screen shots. Our final dataset contains 200 screen shots and 2,804 GUI elements.    

Then we manually inspected the selected sample. For each frame, we identified all visible GUI elements and collected their information. First, we classified them into three types: \code{Text} (e.g. captions of GUI elements, displayed strings), \code{Icon} (an image or drawing that can invoke a functionality), and \code{Comb} (combinations of text labels and icons, i.e. a compounded GUI elements). We also recorded their positions, bounds, shapes, and directions (e.g. vertically or horizontally). For example, the first figure in Figure~\ref{fig:detectFlow} is the home screen of \code{Camera 360} running on an iPhone 6 Plus. We can see the three types of element in one single button. The button \code{Camera} is a Comb element which contains an Icon element (looks like a camera) and a Text element (i.e. the word \code{Camera}).

\subsection{Findings}

We performed several analyses on the collected data. Here are the key findings from those analyses.

\paragraph{Distribution of GUI elements' types} 48.3\% of the identified GUI elements are Text, 39.4\% are Icon, and 12.3\% are Comb. This finding suggests that half of GUI elements are simple text. Because current Optical Character Recognition (OCR) techniques can recognize textual items in images with very high accuracy~\cite{???}, we could employ them to recognize text-based GUI elements.

\paragraph{Shapes and directions of icons} 41.8\% of Icon elements have irregular shapes. 21.7\% have rectangle, 9.6\% have circle, and 10.6\% have arrow shapes. 98.1\% of icons are placed horizontally. 

\paragraph{Shapes and directions of compounded elements} Shapes of most of compounded elements are circle (46.7\%) or rectangle (41.3\%). 87\% of them are placed horizontally.

\paragraph{Relative size of GUI elements} We computed the relative size of a GUI element as the ratio between the area of its bounding box and the screen resolution. Figure~\ref{fig:areaRatioExperiment} plots the results separated on element types, screen sizes, and apps. We have three screen sizes: \code{5s}, \code{6}, and \code{6p} respectively indicate the screen size of iPhone 5s (1136 x 640), iPhone 6 (1334 x 750), and iPhone 6 Plus (1920 x 1080). 

As seen in the figure, Text and Icon elements have stable relative size and the larger screen size. For example, in iPhone 5s, most (75\% and more) of those elements have relative size from 0.1\% to 0.4\%. In addition, the smaller their relative size. For example, Text elements have median relative size of 0.2\% in iPhone 5s and 0.15\% in iPhone 6 Plus.

Relative size of Compounded elements is also stable but often much bigger than that of Text and Icon elements. For example, in iPhone 5s, most (75\% and more) of compounded elements have relative size from 1\% to 5\%.  

Our findings suggest several ideas to design the algorithm to detect GUI elements. First, we could employ OCR to detect Text elements. Then, for two other types, we could use size, shape, and direction to detect and distinguish compounded elements from Icon elements. 

sample interaction sequence
, such as:
\begin{itemize}
\item \textbf{Click} Album button
\item \textbf{Select} an album
\item \textbf{Select} an image
\item \textbf{Click} edit icon
\item \textbf{Swipe right} on options list
\item \textbf{Click} Adjust button
\item \textbf{Swipe right} on options list
\item \textbf{Click} Contrast button
\item \textbf{Adjust} level using slider
\item \textbf{Click} Tick
\item \textbf{Click} Save
\end{itemize}


